The Hunt for New Physics at the Large Hadron Collider

The Large Hadron Collider presents an unprecedented opportunity to probe the realm of new physics in the TeV region and shed light on some of the core unresolved issues of particle physics. These include the nature of electroweak symmetry breaking, the origin of mass, the possible constituent of cold dark matter, new sources of CP violation needed to explain the baryon excess in the universe, the possible existence of extra gauge groups and extra matter, and importantly the path Nature chooses to resolve the hierarchy problem - is it supersymmetry or extra dimensions. Many models of new physics beyond the standard model contain a hidden sector which can be probed at the LHC. Additionally, the LHC will be a top factory and accurate measurements of the properties of the top and its rare decays will provide a window to new physics. Further, the LHC could shed light on the origin of neutralino masses if the new physics associated with their generation lies in the TeV region. Finally, the LHC is also a laboratory to test the hypothesis of TeV scale strings and D-brane models. An overview of these possibilities is presented in the spirit that it will serve as a companion to the Technical Design Reports (TDRs) by the particle detector groups ATLAS and CMS to facilitate the test of the new theoretical ideas at the LHC. Which of these ideas stands the test of the LHC data will govern the course of particle physics in the subsequent decades.

==> ED/newcommands.tex <==
%%%% RS-KK

\def\gsim{\,\,\rlap{\raise 3pt\hbox{$>$}}{\lower 3pt\hbox{$\sim$}}\,\,}
\def\lsim{\,\,\rlap{\raise 3pt\hbox{$<$}}{\lower 3pt\hbox{$\sim$}}\,\,}


\renewcommand{\vev}[1]{\langle {#1} \rangle}
\renewcommand{\ord}[1]{\mathcal{O}{(#1)}}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\fb}[1]{{#1}~fb$^{-1}$}
\newcommand{\mP}{{\bar M}_P}

% %%% ADD-LHC

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc}}
\def\etal{{\it et al.}}
%\def\ibid{{\it ibid}.}
\def\mpl{\ifmmode M_{pl}\else $M_{pl}$\fi}
\def\mpl{\ifmmode \overline M_{Pl}\else $\bar M_{Pl}$\fi}
\def\to{\rightarrow}

%%%%%BH

\def\MBH{\mbox{$M_{\rm BH}$}}

%%%% S1Z2

%\def\beq{\begin{equation}}
%\def\eeq{\end{equation}}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray}}

%%%% Higgsless

%%%% RS-Flavor

\def\bm#1{\mbox{\boldmath$#1$\unboldmath}}

%%%%%RSEW


\def\gtrsim{\gsim}

%%%% Radion

\renewcommand{\nc}{\newcommand}

%\nc{\non}{\nonumber}
%\nc{\beq}{\begin{equation}}   \nc{\eeq}{\end{equation}}
%\nc{\bea}{\begin{eqnarray}}   \nc{\eea}{\end{eqnarray}}
%\nc{\baa}{\begin{array}}      \nc{\eaa}{\end{array}}
%\nc{\bit}{\begin{itemize}}    \nc{\eit}{\end{itemize}}
%\nc{\ben}{\begin{enumerate}}  \nc{\een}{\end{enumerate}}
%\nc{\bce}{\begin{center}}     \nc{\ece}{\end{center}}


==> ref.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% (1) INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{:2008zzm}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
%  ``The ATLAS Experiment at the CERN Large Hadron Collider,''
  JINST {\bf 3} (2008) S08003.
  %%CITATION = JINST,3,S08003;%%
\bibitem{Bayatian:2006zz}
  G.~L.~Bayatian {\it et al.}  [CMS Collaboration],
  ``CMS physics: Technical design report,''
  CERN/LHCC 2006-001 (2006).
  %%CITATION = CMS-TDR-008-1;%%
\bibitem{Spergel:2006hy}
  D.~N.~Spergel {\it et al.}  [WMAP Collaboration],
  %``Wilkinson Microwave Anisotropy Probe (WMAP) three year results:
  %Implications for cosmology,''
  Astrophys.\ J.\ Suppl.\  {\bf 170}, 377 (2007).
  %%CITATION = APJSA,170,377;%%
\bibitem{Komatsu:2008hk}
  E.~Komatsu {\it et al.}  [WMAP Collaboration],
  %``Five-Year Wilkinson Microwave Anisotropy Probe (WMAP\altaffilmark 1 )
  %Observations:Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 180}, 330 (2009).
  %%CITATION = APJSA,180,330;%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% (2) SUSY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{Ramond:1971gb}
  P.~Ramond,
  %``Dual Theory for Free Fermions,''
  Phys.\ Rev.\  D {\bf 3}, 2415 (1971).
  %%CITATION = PHRVA,D3,2415;%%
\bibitem{Golfand:1971iw}
  Yu.~A.~Golfand and E.~P.~Likhtman,
  %``Extension of the Algebra of Poincare Group Generators and Violation of p
  %Invariance,''
  JETP Lett.\  {\bf 13}, 323 (1971)
  [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 13}, 452 (1971)].
  %%CITATION = ZFPRA,13,452;%%
\bibitem{Volkov:1972jx}
  D.~V.~Volkov and V.~P.~Akulov,
  %``Possible universal neutrino interaction,''
  JETP Lett.\  {\bf 16} (1972) 438
  [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 16} (1972) 621].
  %%CITATION = ZFPRA,16,621;%%
\bibitem{Wess:1973kz}
  J.~Wess and B.~Zumino,
  %``A Lagrangian Model Invariant Under Supergauge Transformations,''
  Phys.\ Lett.\  B {\bf 49}, 52 (1974).
  %%CITATION = PHLTA,B49,52;%%
\bibitem{Wess:1974tw}
  J.~Wess and B.~Zumino,
  %``Supergauge Transformations in Four-Dimensions,''
  Nucl.\ Phys.\  B {\bf 70}, 39 (1974).
  %%CITATION = NUPHA,B70,39;%%
\bibitem{Lafaye:2007vs}
  R.~Lafaye, T.~Plehn, M.~Rauch and D.~Zerwas,
  %``Measuring Supersymmetry,''
  Eur.\ Phys.\ J.\  C {\bf 54}, 617 (2008).
  %%CITATION = EPHJA,C54,617;%%
\bibitem{Bechtle:2005vt}
  P.~Bechtle, K.~Desch, W.~Porod and P.~Wienemann,
  %``Determination of MSSM parameters from LHC and ILC observables in a  global
  %fit,''
  Eur.\ Phys.\ J.\  C {\bf 46}, 533 (2006).
  %%CITATION = EPHJA,C46,533;%%
\bibitem{Iliopoulos:1974zv}
  J.~Iliopoulos and B.~Zumino,
  %``Broken Supergauge Symmetry And Renormalization,''
  Nucl.\ Phys.\  B {\bf 76}, 310 (1974).
  %%CITATION = NUPHA,B76,310;%%
\bibitem{Grisaru:1979wc}
  M.~T.~Grisaru, W.~Siegel and M.~Rocek,
  %``Improved Methods For Supergraphs,''
  Nucl.\ Phys.\  B {\bf 159}, 429 (1979).
  %%CITATION = NUPHA,B159,429;%%
\bibitem{Dimopoulos:1981zb}
  S.~Dimopoulos and H.~Georgi,
  %``Softly Broken Supersymmetry And SU(5),''
  Nucl.\ Phys.\  B {\bf 193}, 150 (1981).
  %%CITATION = NUPHA,B193,150;%%
\bibitem{Sakai:1981gr}
  N.~Sakai,
  %``Naturalness In Supersymmetric Guts,''
  Z.\ Phys.\  C {\bf 11}, 153 (1981).
  %%CITATION = ZEPYA,C11,153;%%
\bibitem{Girardello:1981wz}
  L.~Girardello and M.~T.~Grisaru,
  %``Soft Breaking Of Supersymmetry,''
  Nucl.\ Phys.\  B {\bf 194}, 65 (1982).
  %%CITATION = NUPHA,B194,65;%%
\bibitem{Nath:1975nj}
  P.~Nath and R.~L.~Arnowitt,
  %``Generalized Supergauge Symmetry As A New Framework For Unified Gauge
  %Theories,''
  Phys.\ Lett.\  B {\bf 56}, 177 (1975).
  %%CITATION = PHLTA,B56,177;%%
\bibitem{Arnowitt:1975xg}
  R.~L.~Arnowitt, P.~Nath and B.~Zumino,
  %``Superfield Densities And Action Principle In Curved Superspace,''
  Phys.\ Lett.\  B {\bf 56}, 81 (1975).
  %%CITATION = PHLTA,B56,81;%%
\bibitem{Freedman:1976xh}
  D.~Z.~Freedman, P.~van Nieuwenhuizen and S.~Ferrara,
  %``Progress Toward A Theory Of Supergravity,''
  Phys.\ Rev.\  D {\bf 13}, 3214 (1976).
  %%CITATION = PHRVA,D13,3214;%%
\bibitem{Deser:1976eh}
  S.~Deser and B.~Zumino,
  %``Consistent Supergravity,''
  Phys.\ Lett.\  B {\bf 62}, 335 (1976).
  %%CITATION = PHLTA,B62,335;%%
\bibitem{Chamseddine:1982jx}
  A.~H.~Chamseddine, R.~L.~Arnowitt and P.~Nath,
  %``Locally Supersymmetric Grand Unification,''
  Phys.\ Rev.\ Lett.\  {\bf 49} (1982) 970.
  %%CITATION = PRLTA,49,970;%%
\bibitem{Cremmer:1982wb}
  E.~Cremmer, S.~Ferrara, L.~Girardello and A.~Van Proeyen,
%``Yang-Mills Theories With Local Supersymmetry: Lagrangian, Transformation
  %Laws And Superhiggs Effect,''
  Nucl.\ Phys.\  B {\bf 212} (1983) 413.
  %%CITATION = NUPHA,B212,413;%%
\bibitem{Nath:1983fp}
  P.~Nath, R.~L.~Arnowitt and A.~H.~Chamseddine,
  ``Applied N=1 Supergravity,'' World Scientific,1984.
  %%CITATION = NUB-2613;%%
\bibitem{Barbieri:1982eh}
  R.~Barbieri, S.~Ferrara and C.~A.~Savoy,
  %``Gauge Models With Spontaneously Broken Local Supersymmetry,''
  Phys.\ Lett.\  B {\bf 119} (1982) 343.
  %%CITATION = PHLTA,B119,343;%%
\bibitem{Hall:1983iz}
  L.~J.~Hall, J.~D.~Lykken and S.~Weinberg,
  %``Supergravity As The Messenger Of Supersymmetry Breaking,''
  Phys.\ Rev.\  D {\bf 27} (1983) 2359.
  %%CITATION = PHRVA,D27,2359;%%
\bibitem{Nath:1983aw}
  P.~Nath, R.~L.~Arnowitt and A.~H.~Chamseddine,
  %``Gauge Hierarchy In Supergravity Guts,''
  Nucl.\ Phys.\  B {\bf 227} (1983) 121.
  %%CITATION = NUPHA,B227,121;%%
\bibitem{Nilles:1982ik}
  H.~P.~Nilles,
  %``Dynamically Broken Supergravity And The Hierarchy Problem,''
  Phys.\ Lett.\  B {\bf 115}, 193 (1982).
  %%CITATION = PHLTA,B115,193;%%
\bibitem{Ferrara:1982qs}
  S.~Ferrara, L.~Girardello and H.~P.~Nilles,
  %``Breakdown Of Local Supersymmetry Through Gauge Fermion Condensates,''
  Phys.\ Lett.\  B {\bf 125}, 457 (1983).
  %%CITATION = PHLTA,B125,457;%%
\bibitem{Giudice:1988yz}
  G.~F.~Giudice and A.~Masiero,
  %``A Natural Solution to the mu Problem in Supergravity Theories,''
  Phys.\ Lett.\  B {\bf 206} (1988) 480.
  %%CITATION = PHLTA,B206,480;%%
\bibitem{Dine:1995ag}
  M.~Dine, A.~E.~Nelson, Y.~Nir and Y.~Shirman,
  %``New tools for low-energy dynamical supersymmetry breaking,''
  Phys.\ Rev.\  D {\bf 53} (1996) 2658.
%  [arXiv:hep-ph/9507378].
  %%CITATION = PHRVA,D53,2658;%%
\bibitem{Giudice:1998bp}
  G.~F.~Giudice and R.~Rattazzi,
  %``Theories with gauge-mediated supersymmetry breaking,''
  Phys.\ Rept.\  {\bf 322} (1999) 419.
%  [arXiv:hep-ph/9801271].
  %%CITATION = PRPLC,322,419;%%
\bibitem{Randall:1998uk}
  L.~Randall and R.~Sundrum,
  %``Out of this world supersymmetry breaking,''
  Nucl.\ Phys.\  B {\bf 557} (1999) 79.
%  [arXiv:hep-th/9810155].
  %%CITATION = NUPHA,B557,79;%%
\bibitem{Giudice:1998xp}
  G.~F.~Giudice, M.~A.~Luty, H.~Murayama and R.~Rattazzi,
  %``Gaugino Mass without Singlets,''
  JHEP {\bf 9812} (1998) 027.
  %%CITATION = JHEPA,9812,027;%%
\bibitem{Nilles:1983ge}
  H.~P.~Nilles,
  %``Supersymmetry, Supergravity And Particle Physics,''
  Phys.\ Rept.\  {\bf 110}, 1 (1984).
  %%CITATION = PRPLC,110,1;%%
\bibitem{Haber:1984rc}
  H.~E.~Haber and G.~L.~Kane,
  %``The Search For Supersymmetry: Probing Physics Beyond The Standard Model,''
  Phys.\ Rept.\  {\bf 117} (1985) 75.
  %%CITATION = PRPLC,117,75;%%
\bibitem{Martin:1997ns}
  S.~P.~Martin,
%  ``A Supersymmetry Primer,''
  arXiv:hep-ph/9709356.
  %%CITATION = HEP-PH/9709356;%%
\bibitem{Nath:2003zs}
  P.~Nath,
  %``Twenty years of SUGRA,''
  arXiv:hep-ph/0307123.
  %%CITATION = HEP-PH/0307123;%%
\bibitem{Baer:2006rs}
  H.~Baer and X.~Tata,
  ``Weak scale supersymmetry: From superfields to scattering events,''
%\href{http://www.slac.stanford.edu/spires/find/hep/www?irn=6927297}{SPIRES entry}
{\it  Cambridge, UK: Univ. Pr. (2006) 537 p}
\bibitem{Drees:2004jm}
  M.~Drees, R.~Godbole and P.~Roy,
%  ``Theory and phenomenology of sparticles: An account of four-dimensional N=1
%  supersymmetry in high energy physics,''
%\href{http://www.slac.stanford.edu/spires/find/hep/www?irn=6240364}{SPIRES entry}
   {\it  Hackensack, USA: World Scientific (2004) 555 p};
\bibitem{pierrebook} P.~Binetruy, ``Supersymmetry,'' {\it Oxford, UK
(2007).}
\bibitem{Feldman:2007zn}
  D.~Feldman, Z.~Liu and P.~Nath,
  %``The Landscape of Sparticle Mass Hierarchies and Their Signature Space at
  %the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 99}, 251802 (2007)
  [Erratum-ibid.\  {\bf 100}, 069902 (2008)].
  %%CITATION = PRLTA,99,251802;%%
\bibitem{Inoue:1982pi}
  K.~Inoue, A.~Kakuto, H.~Komatsu and S.~Takeshita,
  %``Aspects Of Grand Unified Models With Softly Broken Supersymmetry,''
  Prog.\ Theor.\ Phys.\  {\bf 68}, 927 (1982)
  [Erratum-ibid.\  {\bf 70}, 330 (1983)].
  %%CITATION = PTPKA,68,927;%%
\bibitem{Ibanez:1982fr}
  L.~E.~Ibanez and G.~G.~Ross,
  %``SU(2)-L X U(1) Symmetry Breaking As A Radiative Effect Of Supersymmetry
  %Breaking In Guts,''
  Phys.\ Lett.\  B {\bf 110}, 215 (1982).
  %%CITATION = PHLTA,B110,215;%%
\bibitem{AlvarezGaume:1983gj}
  L.~Alvarez-Gaume, J.~Polchinski and M.~B.~Wise,
  %``Minimal Low-Energy Supergravity,''
  Nucl.\ Phys.\  B {\bf 221}, 495 (1983).
  %%CITATION = NUPHA,B221,495;%%
\bibitem{Machacek:1983tz}
  M.~E.~Machacek and M.~T.~Vaughn,
  %``Two Loop Renormalization Group Equations In A General Quantum Field Theory.
  %1. Wave Function Renormalization,''
  Nucl.\ Phys.\  B {\bf 222}, 83 (1983).
  %%CITATION = NUPHA,B222,83;%%
\bibitem{Machacek:1983fi}
  M.~E.~Machacek and M.~T.~Vaughn,
  %``Two Loop Renormalization Group Equations In A General Quantum Field Theory.
  %2. Yukawa Couplings,''
  Nucl.\ Phys.\  B {\bf 236}, 221 (1984).
  %%CITATION = NUPHA,B236,221;%%
\bibitem{Machacek:1984zw}
  M.~E.~Machacek and M.~T.~Vaughn,
  %``Two Loop Renormalization Group Equations In A General Quantum Field Theory.
  %3. Scalar Quartic Couplings,''
  Nucl.\ Phys.\  B {\bf 249}, 70 (1985).
  %%CITATION = NUPHA,B249,70;%%
\bibitem{Martin:1993yx}
  S.~P.~Martin and M.~T.~Vaughn,
  %``Regularization dependence of running couplings in softly broken
  %supersymmetry,''
  Phys.\ Lett.\  B {\bf 318}, 331 (1993).
  %%CITATION = PHLTA,B318,331;%%
\bibitem{Martin:1993zk}
  S.~P.~Martin and M.~T.~Vaughn,
  %``Two Loop Renormalization Group Equations For Soft Supersymmetry Breaking
  %Couplings,''
  Phys.\ Rev.\  D {\bf 50}, 2282 (1994)
  [Erratum-ibid.\  D {\bf 78}, 039903 (2008)].
  %%CITATION = PHRVA,D50,2282;%%
\bibitem{Jack:1994rk}
  I.~Jack, D.~R.~T.~Jones, S.~P.~Martin, M.~T.~Vaughn and Y.~Yamada,
  %``Decoupling of the epsilon scalar mass in softly broken supersymmetry,''
  Phys.\ Rev.\  D {\bf 50}, 5481 (1994).
  %%CITATION = PHRVA,D50,5481;%%
\bibitem{Weinberg:1982tp}
  S.~Weinberg,
  %``Upper Bound On Gauge Fermion Masses,''
  Phys.\ Rev.\ Lett.\  {\bf 50}, 387 (1983).
  %%CITATION = PRLTA,50,387;%%
\bibitem{Arnowitt:1983ah}
  R.~L.~Arnowitt, A.~H.~Chamseddine and P.~Nath,
  %``Masses Of Superpartners Of Quarks, Leptons, And Gauge Mesons In
  %Supergravity Grand Unified Theories,''
  Phys.\ Rev.\ Lett.\  {\bf 50}, 232 (1983).
  %%CITATION = PRLTA,50,232;%%
\bibitem{Chamseddine:1983eg}
  A.~H.~Chamseddine, P.~Nath and R.~L.~Arnowitt,
  %``Experimental Signals For Supersymmetric Decays Of The W And Z Bosons,''
  Phys.\ Lett.\  B {\bf 129}, 445 (1983)
  [Erratum-ibid.\  B {\bf 132}, 467 (1983)].
  %%CITATION = PHLTA,B129,445;%%
\bibitem{Dicus:1983fe}
  D.~A.~Dicus, S.~Nandi, W.~W.~Repko and X.~Tata,
  %``Electron - Positron Annihilation Cross-Section In SU(2)-L X U(1)
  %Supergravity,''
  Phys.\ Rev.\ Lett.\  {\bf 51}, 1030 (1983)
  [Erratum-ibid.\  {\bf 51}, 1813 (1983)].
  %%CITATION = PRLTA,51,1030;%%
\bibitem{Dicus:1983fd}
  D.~A.~Dicus, S.~Nandi, W.~W.~Repko and X.~Tata,
  %``Electron Spectra From Wino Decay At The Anti-P P Collider,''
  Phys.\ Rev.\  D {\bf 29}, 67 (1984).
  %%CITATION = PHRVA,D29,67;%%
\bibitem{Dicus:1983aa}
  D.~A.~Dicus, S.~Nandi, W.~W.~Repko and X.~Tata,
  %``Lepton Pair Production As A Signature Of Supersymmetry,''
  Phys.\ Rev.\  D {\bf 29}, 1317 (1984).
  %%CITATION = PHRVA,D29,1317;%%
\bibitem{Dicus:1983cb}
  D.~A.~Dicus, S.~Nandi and X.~Tata,
  %``W Decay In Supergravity Guts,''
  Phys.\ Lett.\  B {\bf 129}, 451 (1983)
  [Erratum-ibid.\  B {\bf 145}, 448 (1984)].
  %%CITATION = PHLTA,B129,451;%%
\bibitem{Frere:1983dd}
  J.~M.~Frere and G.~L.~Kane,
  %``On The Possibility Of Finding Light Uncolored Supersymmetric Partners At
  %Present And Future Machines,''
  Nucl.\ Phys.\  B {\bf 223}, 331 (1983).
  %%CITATION = NUPHA,B223,331;%%
\bibitem{Ellis:1983er}
  J.~R.~Ellis, J.~M.~Frere, J.~S.~Hagelin, G.~L.~Kane and S.~T.~Petcov,
  %``Search For Neutral Gauge Fermions In E+ E- Annihilation,''
  Phys.\ Lett.\  B {\bf 132}, 436 (1983).
  %%CITATION = PHLTA,B132,436;%%
\bibitem{Dimopoulos:1981yj}
  S.~Dimopoulos, S.~Raby and F.~Wilczek,
  %``Supersymmetry And The Scale Of Unification,''
  Phys.\ Rev.\  D {\bf 24}, 1681 (1981).
  %%CITATION = PHRVA,D24,1681;%%
\bibitem{Ellis:1990zq}
  J.~R.~Ellis, S.~Kelley and D.~V.~Nanopoulos,
  %``Precision Lep Data, Supersymmetric Guts And String Unification,''
  Phys.\ Lett.\  B {\bf 249}, 441 (1990).
  %%CITATION = PHLTA,B249,441;%%
\bibitem{Ellis:1990wk}
  J.~R.~Ellis, S.~Kelley and D.~V.~Nanopoulos,
  %``Probing the desert using gauge coupling unification,''
  Phys.\ Lett.\  B {\bf 260}, 131 (1991).
  %%CITATION = PHLTA,B260,131;%%
\bibitem{Amaldi:1991cn}
  U.~Amaldi, W.~de Boer and H.~Furstenau,
  %``Comparison of grand unified theories with electroweak and strong coupling
  %constants measured at LEP,''
  Phys.\ Lett.\  B {\bf 260}, 447 (1991).
  %%CITATION = PHLTA,B260,447;%%
\bibitem{Langacker:1991an}
  P.~Langacker and M.~x.~Luo,
  %``Implications of precision electroweak experiments for $M_t$, $\rho_{0}$,
  %$\sin^2\theta_W$ and grand unification,''
  Phys.\ Rev.\  D {\bf 44}, 817 (1991).
  %%CITATION = PHRVA,D44,817;%%
\bibitem{Anselmo:1991uu}
  F.~Anselmo, L.~Cifarelli, A.~Peterman and A.~Zichichi,
  %``The Effective experimental constraints on M (susy) and M (gut),''
  Nuovo Cim.\  A {\bf 104}, 1817 (1991).
  %%CITATION = NUCIA,104A,1817;%%
\bibitem{Arnowitt:1992aq}
  R.~L.~Arnowitt and P.~Nath,
  %``SUSY mass spectrum in SU(5) supergravity grand unification,''
  Phys.\ Rev.\ Lett.\  {\bf 69} (1992) 725.
  %%CITATION = PRLTA,69,725;%%
\bibitem{Ross:1992tz}
  G.~G.~Ross and R.~G.~Roberts,
  %``Minimal supersymmetric unification predictions,''
  Nucl.\ Phys.\  B {\bf 377}, 571 (1992).
  %%CITATION = NUPHA,B377,571;%%
\bibitem{Barger:1993gh}
  V.~D.~Barger, M.~S.~Berger and P.~Ohmann,
  %``The Supersymmetric particle spectrum,''
  Phys.\ Rev.\  D {\bf 49}, 4908 (1994).
  %%CITATION = PHRVA,D49,4908;%%
\bibitem{Kane:1993td}
  G.~L.~Kane, C.~F.~Kolda, L.~Roszkowski and J.~D.~Wells,
  %``Study of constrained minimal supersymmetry,''
  Phys.\ Rev.\  D {\bf 49}, 6173 (1994).
  %%CITATION = PHRVA,D49,6173;%%
\bibitem{Baer:1994zt}
  H.~Baer, M.~Drees, C.~Kao, M.~Nojiri and X.~Tata,
  %``Supercollider Signatures Of Supergravity Models With Yukawa Unification,''
  Phys.\ Rev.\  D {\bf 50} (1994) 2148.
  %%CITATION = PHRVA,D50,2148;%%
\bibitem{Chan:1997bi}
  K.~L.~Chan, U.~Chattopadhyay and P.~Nath,
  %``Naturalness, weak scale supersymmetry and the prospect for the  observation
  %of supersymmetry at the Tevatron and at the LHC,''
  Phys.\ Rev.\  D {\bf 58}, 096004 (1998).
  %%CITATION = PHRVA,D58,096004;%%
\bibitem{Feng:1999mn}
  J.~L.~Feng, K.~T.~Matchev and T.~Moroi,
  %``Multi-TeV scalars are natural in minimal supergravity,''
  Phys.\ Rev.\ Lett.\  {\bf 84}, 2322 (2000).
  %%CITATION = PRLTA,84,2322;%%
\bibitem{Baer:2003wx}
  H.~Baer, C.~Balazs, A.~Belyaev, T.~Krupovnickas and X.~Tata,
  %``Updated reach of the CERN LHC and constraints from relic density, $b \to s
  %\gamma$ and a($\mu$) in the mSUGRA model,''
  JHEP {\bf 0306}, 054 (2003).
  %%CITATION = JHEPA,0306,054;%%
\bibitem{Lahanas:2003bh}
  A.~B.~Lahanas, N.~E.~Mavromatos and D.~V.~Nanopoulos,
  %``WMAPing the universe: Supersymmetry, dark matter, dark energy, proton
  %decay and collider physics,''
  Int.\ J.\ Mod.\ Phys.\  D {\bf 12}, 1529 (2003).
  %%CITATION = IMPAE,D12,1529;%%
\bibitem{Martin:1993ft}
  S.~P.~Martin and P.~Ramond,
  %``Sparticle spectrum constraints,''
  Phys.\ Rev.\  D {\bf 48}, 5365 (1993).
  %%CITATION = PHRVA,D48,5365;%%
\bibitem{Bennett:2002jb}
  G.~W.~Bennett {\it et al.}  [Muon g-2 Collaboration],
  %``Measurement of the Positive Muon Anomalous Magnetic Moment to 0.7 ppm,''
  Phys.\ Rev.\ Lett.\  {\bf 89}, 101804 (2002)
  [Erratum-ibid.\  {\bf 89}, 129903 (2002)].
  %%CITATION = PRLTA,89,101804;%%
\bibitem{Yuan:1984ww}
  T.~C.~Yuan, R.~L.~Arnowitt, A.~H.~Chamseddine and P.~Nath,
  %``Supersymmetric Electroweak Effects On G-2 (Mu),''
  Z.\ Phys.\  C {\bf 26}, 407 (1984).
  %%CITATION = ZEPYA,C26,407;%%
\bibitem{Kosower:1983yw}
  D.~A.~Kosower, L.~M.~Krauss and N.~Sakai,
  %``Low-Energy Supergravity And The Anomalous Magnetic Moment Of The Muon,''
  Phys.\ Lett.\  B {\bf 133}, 305 (1983).
  %%CITATION = PHLTA,B133,305;%%
\bibitem{Lopez:1993vi}
  J.~L.~Lopez, D.~V.~Nanopoulos and X.~Wang,
  %``Large (G-2)-Mu In SU(5) X U(1) Supergravity Models,''
  Phys.\ Rev.\  D {\bf 49}, 366 (1994).
  %%CITATION = PHRVA,D49,366;%%
\bibitem{Chattopadhyay:1995ae}
  U.~Chattopadhyay and P.~Nath,
  %``Probing supergravity grand unification in the Brookhaven g-2 experiment,''
  Phys.\ Rev.\  D {\bf 53}, 1648 (1996).
\bibitem{Moroi:1995yh}
  T.~Moroi,
  %``The Muon Anomalous Magnetic Dipole Moment in the Minimal Supersymmetric
  %Standard Model,''
  Phys.\ Rev.\  D {\bf 53}, 6565 (1996)
  [Erratum-ibid.\  D {\bf 56}, 4424 (1997)].
  %%CITATION = PHRVA,D53,6565;%%
\bibitem{Davier:2009zi}
  M.~Davier, A.~Hoecker, B.~Malaescu, C.~Z.~Yuan and Z.~Zhang,
  %``Reevaluation of the hadronic contribution to the muon magnetic anomaly
  %using new e+e- -> pi+pi- cross section data from BABAR,''
  arXiv:0908.4300 [hep-ph].
  %%CITATION = ARXIV:0908.4300;%%
\bibitem{Feng:2001tr}
  J.~L.~Feng and K.~T.~Matchev,
  %``Supersymmetry and the anomalous anomalous magnetic moment of the muon,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 3480 (2001).
  %%CITATION = PRLTA,86,3480;%%
\bibitem{Baltz:2001ts}
  E.~A.~Baltz and P.~Gondolo,
  %``Implications of muon anomalous magnetic moment for supersymmetric dark
  %matter,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 5004 (2001).
  %%CITATION = PRLTA,86,5004;%%
\bibitem{Everett:2001tq}
  L.~L.~Everett, G.~L.~Kane, S.~Rigolin and L.~T.~Wang,
  %``Implications of muon g-2 for supersymmetry and for discovering
  %superpartners directly,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 3484 (2001).
  %%CITATION = PRLTA,86,3484;%%
\bibitem{Chattopadhyay:2001vx}
  U.~Chattopadhyay and P.~Nath,
  %``Upper limits on sparticle masses from g-2 and the possibility for
  %discovery of SUSY at colliders and in dark matter searches,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 5854 (2001).
  %%CITATION = PRLTA,86,5854;%%
\bibitem{Ibrahim:2001ym}
  T.~Ibrahim, U.~Chattopadhyay and P.~Nath,
  %``Constraints on explicit CP violation from the Brookhaven muon g-2
  %experiment,''
  Phys.\ Rev.\  D {\bf 64}, 016010 (2001).
  %%CITATION = PHRVA,D64,016010;%%
\bibitem{Ellis:2001yu}
  J.~R.~Ellis, D.~V.~Nanopoulos and K.~A.~Olive,
  %``Combining the muon anomalous magnetic moment with other constraints on  the
  %CMSSM,''
  Phys.\ Lett.\  B {\bf 508}, 65 (2001).
  %%CITATION = PHLTA,B508,65;%%
\bibitem{Arnowitt:2001be}
  R.~L.~Arnowitt, B.~Dutta, B.~Hu and Y.~Santoso,
  %``Muon g-2, dark matter detection and accelerator physics,''
  Phys.\ Lett.\  B {\bf 505}, 177 (2001).
  %%CITATION = PHLTA,B505,177;%%
\bibitem{Martin:2001st}
  S.~P.~Martin and J.~D.~Wells,
  %``Muon anomalous magnetic dipole moment in supersymmetric theories,''
  Phys.\ Rev.\  D {\bf 64}, 035003 (2001).
  %%CITATION = PHRVA,D64,035003;%%
\bibitem{Baer:2001kn}
  H.~Baer, C.~Balazs, J.~Ferrandis and X.~Tata,
  %``Impact of muon anomalous magnetic moment on supersymmetric models,''
  Phys.\ Rev.\  D {\bf 64}, 035004 (2001).
  %%CITATION = PHRVA,D64,035004;%%
\bibitem{Bertolini:1986th}
  S.~Bertolini, F.~Borzumati and A.~Masiero,
  %``QCD Enhancement Of Radiative B Decays,''
  Phys.\ Rev.\ Lett.\  {\bf 59}, 180 (1987).
  %%CITATION = PRLTA,59,180;%%
\bibitem{Borzumati:1999qt}
  F.~Borzumati, C.~Greub, T.~Hurth and D.~Wyler,
  %``Gluino contribution to radiative B decays: Organization of QCD  corrections
  %and leading order results,''
  Phys.\ Rev.\  D {\bf 62}, 075005 (2000).
  %%CITATION = PHRVA,D62,075005;%%
\bibitem{Gomez:2006uv}
  M.~E.~Gomez, T.~Ibrahim, P.~Nath and S.~Skadhauge,
  %``An improved analysis of b --> s gamma in supersymmetry,''
  Phys.\ Rev.\  D {\bf 74}, 015015 (2006).
  %%CITATION = PHRVA,D74,015015;%%
\bibitem{Degrassi:2006eh}
  G.~Degrassi, P.~Gambino and P.~Slavich,
  %``QCD corrections to radiative B decays in the MSSM with minimal flavor
  %violation,''
  Phys.\ Lett.\  B {\bf 635}, 335 (2006).
  %%CITATION = PHLTA,B635,335;%%
\bibitem{Misiak:2006zs}
  M.~Misiak {\it et al.},
  %``The first estimate of B(anti-B --> X/s gamma) at O(alpha(s)**2),''
  Phys.\ Rev.\ Lett.\  {\bf 98} (2007) 022002.
%  [arXiv:hep-ph/0609232].
  %%CITATION = PRLTA,98,022002;%%
\bibitem{Barberio:2008fa}
  E.~Barberio {\it et al.}  [Heavy Flavor Averaging Group],
  %``Averages of $b-$hadron and $c-$hadron Properties at the End of 2007,''
  arXiv:0808.1297 [hep-ex].
  %%CITATION = ARXIV:0808.1297;%%
\bibitem{Chen:2009cw}
  N.~Chen, D.~Feldman, Z.~Liu and P.~Nath,
  %``SUSY and Higgs Signatures Implied by Cancellations in $b\to s\gamma$,''
  arXiv:0911.0217 [hep-ph].
  %%CITATION = ARXIV:0911.0217;%%
\bibitem{Goldberg:1983nd}
  H.~Goldberg,
  %``Constraint on the photino mass from cosmology,''
  Phys.\ Rev.\ Lett.\  {\bf 50}, 1419 (1983)
  [Erratum-ibid.\  {\bf 103}, 099905 (2009)].
  %%CITATION = PRLTA,50,1419;%%
\bibitem{Ellis:1983wd}
  J.~R.~Ellis, J.~S.~Hagelin, D.~V.~Nanopoulos and M.~Srednicki,
  %``Search For Supersymmetry At The Anti-P P Collider,''
  Phys.\ Lett.\  B {\bf 127}, 233 (1983).
  %%CITATION = PHLTA,B127,233;%%
\bibitem{Feldman:2008hs}
  D.~Feldman, Z.~Liu and P.~Nath,
  %``Sparticles at the LHC,''
  JHEP {\bf 0804}, 054 (2008).
%  [arXiv:0802.4085 [hep-ph]].
  %%CITATION = JHEPA,0804,054;%%
\bibitem{Ellis:1985jn}
  J.~R.~Ellis, K.~Enqvist, D.~V.~Nanopoulos and K.~Tamvakis,
  %``Gaugino Masses And Grand Unification,''
  Phys.\ Lett.\  B {\bf 155}, 381 (1985).
  %%CITATION = PHLTA,B155,381;%%
\bibitem{Ellis:1985jn}
  J.R.~Ellis, K.~Enqvist, D.V.~Nanopoulos and K.~Tamvakis,
  %``Gaugino Masses And Grand Unification,''
  Phys.\ Lett.\  B {\bf 155}, 381 (1985);
  %%CITATION = PHLTA,B155,381;%%
\bibitem{Drees:1985bx}
  M.~Drees,
  %``Phenomenological Consequences Of N=1 Supergravity Theories With Nonminimal
  %Kinetic Energy Terms For Vector Superfields,''
  Phys.\ Lett.\  B {\bf 158}, 409 (1985).
\bibitem{Anderson:1996bg}
  G.~Anderson, C.~H.~Chen, J.~F.~Gunion, J.~D.~Lykken, T.~Moroi and Y.~Yamada,
  %``Motivations for and implications of non-universal GUT-scale boundary
  %conditions for soft SUSY-breaking parameters,''
%{\it In the Proceedings of 1996 DPF / DPB Summer Study on New
%Directions for High-Energy Physics (Snowmass 96), Snowmass,
%Colorado, 25 Jun - 12 Jul 1996, pp SUP107}
  [arXiv:hep-ph/9609457].
  %%CITATION = ECONF,C960625,SUP107;%%
\bibitem{Nath:1997qm}
  P.~Nath and R.~L.~Arnowitt,
  %``Non-universal soft SUSY breaking and dark matter,''
  Phys.\ Rev.\  D {\bf 56}, 2820 (1997);
%  [arXiv:hep-ph/9701301].
  %%CITATION = PHRVA,D56,2820;%%
\bibitem{Arnowitt:2001yh}
  R.~L.~Arnowitt, B.~Dutta and Y.~Santoso,
  %``Coannihilation effects in supergravity and D-brane models,''
  Nucl.\ Phys.\  B {\bf 606}, 59 (2001).
  %%CITATION = NUPHA,B606,59;%%
\bibitem{Ellis:2002iu}
  J.~R.~Ellis, T.~Falk, K.~A.~Olive and Y.~Santoso,
  %``Exploration of the MSSM with Non-Universal Higgs Masses,''
  Nucl.\ Phys.\  B {\bf 652}, 259 (2003).
  %%CITATION = NUPHA,B652,259;%%
\bibitem{Cerdeno:2004zj}
  D.~G.~Cerdeno and C.~Munoz,
  %``Neutralino dark matter in supergravity theories with non-universal  scalar
  %and gaugino masses,''
  JHEP {\bf 0410}, 015 (2004).
\bibitem{Corsetti:2000yq}
  A.~Corsetti and P.~Nath,
  %``Gaugino Mass Nonuniversality and Dark Matter in SUGRA, Strings and D Brane
  %Models,''
  Phys.\ Rev.\  D {\bf 64}, 125010 (2001).
  %%CITATION = PHRVA,D64,125010;%%
\bibitem{Chattopadhyay:2001mj}
  U.~Chattopadhyay and P.~Nath,
  %``b - tau unification, g(mu)-2, the b --> s + gamma constraint and
  %nonuniversalities,''
  Phys.\ Rev.\  D {\bf 65}, 075009 (2002).
  %%CITATION = PHRVA,D65,075009;%%
\bibitem{BirkedalHansen:2001is}
  A.~Birkedal-Hansen and B.~D.~Nelson,
  %``The role of Wino content in neutralino dark matter,''
  Phys.\ Rev.\  D {\bf 64}, 015008 (2001).
%  [arXiv:hep-ph/0102075].
  %%CITATION = PHRVA,D64,015008;%%
\bibitem{BirkedalHansen:2002am}
  A.~Birkedal-Hansen and B.~D.~Nelson,
  %``Relic neutralino densities and detection rates with nonuniversal gaugino
  %masses,''
  Phys.\ Rev.\  D {\bf 67}, 095006 (2003).
%  [arXiv:hep-ph/0211071].
  %%CITATION = PHRVA,D67,095006;%%
\bibitem{Chattopadhyay:2003yk}
  U.~Chattopadhyay and D.~P.~Roy,
  %``Higgsino dark matter in a SUGRA model with nonuniversal gaugino masses,''
  Phys.\ Rev.\  D {\bf 68}, 033010 (2003).
  %%CITATION = PHRVA,D68,033010;%%
\bibitem{Belanger:2004ag}
  G.~Belanger, F.~Boudjema, A.~Cottrant, A.~Pukhov and A.~Semenov,
  %``WMAP constraints on SUGRA models with non-universal gaugino masses and
  %prospects for direct detection,''
  Nucl.\ Phys.\  B {\bf 706}, 411 (2005).
  %%CITATION = NUPHA,B706,411;%%
\bibitem{Gogoladze:2008dk}
  I.~Gogoladze, R.~Khalid, N.~Okada and Q.~Shafi,
  %``Soft Probes of SU(5) Unification,''
  Phys.\ Rev.\  D {\bf 79}, 095022 (2009).
  %%CITATION = PHRVA,D79,095022;%%
\bibitem{Bhattacharya:2008qu}
  S.~Bhattacharya, A.~Datta and B.~Mukhopadhyaya,
  %``Non-universal gaugino and scalar masses, hadronically quiet trileptons and
  %the Large Hadron Collider,''
  Phys.\ Rev.\  D {\bf 78}, 115018 (2008).
  %%CITATION = PHRVA,D78,115018;%%
\bibitem{Gomez:2009yc}
  M.~E.~Gomez, S.~Lola, P.~Naranjo and J.~Rodriguez-Quintero,
  %``WMAP Dark Matter Constraints on Yukawa Unification with Massive
  %Neutrinos,''
  JHEP {\bf 0904}, 043 (2009).
  %%CITATION = JHEPA,0904,043;%%
\bibitem{Chattopadhyay:2009fr}
  U.~Chattopadhyay, D.~Das and D.~P.~Roy,
  %``Mixed Neutralino Dark Matter in Nonuniversal Gaugino Mass Models,''
  Phys.\ Rev.\  D {\bf 79}, 095013 (2009).
  %%CITATION = PHRVA,D79,095013;%%
\bibitem{Baer:2005bu}
  H.~Baer, A.~Mustafayev, S.~Profumo, A.~Belyaev and X.~Tata,
  %``Direct, indirect and collider detection of neutralino dark matter in SUSY
  %models with non-universal Higgs masses,''
  JHEP {\bf 0507}, 065 (2005).
%  [arXiv:hep-ph/0504001].
  %%CITATION = JHEPA,0507,065;%%
\bibitem{Anderson:1999uia}
  G.~Anderson, H.~Baer, C.~h.~Chen and X.~Tata,
  %``The reach of Fermilab Tevatron upgrades for SU(5) supergravity models  with
  %non-universal gaugino masses,''
  Phys.\ Rev.\  D {\bf 61}, 095005 (2000).
  %%CITATION = PHRVA,D61,095005;%%
\bibitem{Choi:2007ka}
  K.~Choi and H.~P.~Nilles,
  %``The gaugino code,''
  JHEP {\bf 0704}, 006 (2007).
  %%CITATION = JHEPA,0704,006;%%
\bibitem{Altunkaynak:2009tg}
  B.~Altunkaynak, P.~Grajek, M.~Holmes, G.~Kane and B.~D.~Nelson,
  %``Studying Gaugino Mass Unification at the LHC,''
  JHEP {\bf 0904}, 114 (2009).
  %%CITATION = JHEPA,0904,114;%%
\bibitem{Baer:1986vf}
  H.~Baer, K.~Hagiwara and X.~Tata,
  %``Gauginos as a Signal for Supersymmetry at p anti-p Colliders,''
  Phys.\ Rev.\  D {\bf 35}, 1598 (1987).
  %%CITATION = PHRVA,D35,1598;%%
\bibitem{Nath:1987sw}
  P.~Nath and R.~L.~Arnowitt,
  %``Supersymmetric Signals at the Tevatron,''
  Mod.\ Phys.\ Lett.\  A {\bf 2} (1987) 331.
  %%CITATION = MPLAE,A2,331;%%
\bibitem{Dawson:1983fw}
  S.~Dawson, E.~Eichten and C.~Quigg,
  %``Search For Supersymmetric Particles In Hadron - Hadron Collisions,''
  Phys.\ Rev.\  D {\bf 31} (1985) 1581.
  %%CITATION = PHRVA,D31,1581;%%
\bibitem{Feng:2009te}
  J.~L.~Feng, J.~F.~Grivaz and J.~Nachtman,
  %``Searches for Supersymmetry at High-Energy Colliders,''
  arXiv:0903.0046 [hep-ex].
  %%CITATION = ARXIV:0903.0046;%%
\bibitem{Datta:2005vx}
  A.~Datta, G.~L.~Kane and M.~Toharia,
  %``Is it SUSY?,''
  arXiv:hep-ph/0510204.
  %%CITATION = HEP-PH/0510204;%%
\bibitem{Smillie:2005ar}
  J.~M.~Smillie and B.~R.~Webber,
  %``Distinguishing Spins in Supersymmetric and Universal Extra Dimension Models
  %at the Large Hadron Collider,''
  JHEP {\bf 0510} (2005) 069.
  %%CITATION = JHEPA,0510,069;%%
\bibitem{ArkaniHamed:2005px}
  N.~Arkani-Hamed, G.~L.~Kane, J.~Thaler and L.~T.~Wang,
  %``Supersymmetry and the LHC inverse problem,''
  JHEP {\bf 0608} (2006) 070.
%  [arXiv:hep-ph/0512190].
  %%CITATION = JHEPA,0608,070;%%
\bibitem{Altunkaynak:2008ry}
  B.~Altunkaynak, M.~Holmes and B.~D.~Nelson,
  %``Solving the LHC Inverse Problem with Dark Matter Observations,''
  JHEP {\bf 0810} (2008) 013.
%  [arXiv:0804.2899 [hep-ph]].
  %%CITATION = JHEPA,0810,013;%%
\bibitem{Balazs:2009it}
  C.~Balazs and D.~Kahawala,
  %``Stochastic resolution of the LHC inverse problem,''
  arXiv:0904.0128 [hep-ph].
  %%CITATION = ARXIV:0904.0128;%%
\bibitem{Arnowitt:2008bz}
  R.~L.~Arnowitt, B.~Dutta, A.~Gurrola, T.~Kamon, A.~Krislock and D.~Toback,
%  ``Determining the Dark Matter Relic Density in the mSUGRA Stau-Neutralino
%  Co-Annhiliation Region at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 231802 (2008).
%  [arXiv:0802.2968 [hep-ph]].
  %%CITATION = PRLTA,100,231802;%%
\bibitem{Arnowitt:2007nt}
  R.~L.~Arnowitt {\it et al.},
  %``Indirect measurements of the stau - neutralino 1(0) mass difference and
  %mSUGRA in the co-annihilation region of mSUGRA models at the LHC,''
  Phys.\ Lett.\  B {\bf 649}, 73 (2007).
  %%CITATION = PHLTA,B649,73;%%
\bibitem{Arnowitt:2006jq}
  R.~L.~Arnowitt, B.~Dutta, T.~Kamon, N.~Kolev and D.~A.~Toback,
  %``Detection of SUSY in the stau-neutralino coannihilation region at the
  %LHC,''
  Phys.\ Lett.\  B {\bf 639}, 46 (2006).
  %%CITATION = PHLTA,B639,46;%%
\bibitem{Nojiri:2008hy}
  M.~M.~Nojiri, Y.~Shimizu, S.~Okada and K.~Kawagoe,
  %``Inclusive transverse mass analysis for squark and gluino mass
  %determination,''
  JHEP {\bf 0806} (2008) 035.
%  [arXiv:0802.2412 [hep-ph]].
\bibitem{Hubisz:2008gg}
  J.~Hubisz, J.~Lykken, M.~Pierini and M.~Spiropulu,
  %``Missing energy look-alikes with 100 pb$^{-1}$ at the LHC,''
  Phys.\ Rev.\  D {\bf 78} (2008) 075008.
%  [arXiv:0805.2398 [hep-ph]].
  %%CITATION = PHRVA,D78,075008;%%
\bibitem{Baer:2008kc}
  H.~Baer, H.~Prosper and H.~Summy,
  %``Early SUSY discovery at LHC without missing E_T: the role of
  %multi-leptons,''
  Phys.\ Rev.\  D {\bf 77} (2008) 055017.
%  [arXiv:0801.3799 [hep-ph]].
  %%CITATION = PHRVA,D77,055017;%%
\bibitem{Baer:2008ey}
  H.~Baer, A.~Lessa and H.~Summy,
  %``Early SUSY discovery at LHC via sparticle cascade decays to same-sign and
  %multimuon states,''
  Phys.\ Lett.\  B {\bf 674} (2009) 49.
%  [arXiv:0809.4719 [hep-ph]].
  %%CITATION = PHLTA,B674,49;%%
\bibitem{Baer:2009dn}
  H.~Baer, V.~Barger, A.~Lessa and X.~Tata,
  %``Supersymmetry discovery potential of the LHC at $\sqrt{s}=$10 and 14 TeV
  %without and with missing $E_T$,''
  JHEP {\bf 0909}, 063 (2009).
  %%CITATION = JHEPA,0909,063;%%
\bibitem{Edsjo:2009rr}
  J.~Edsjo, E.~Lundstrom, S.~Rydbeck and J.~Sjolin,
  %``Early search for supersymmetric dark matter models at the LHC without
  %missing energy,''
  arXiv:0910.1106 [hep-ph].
  %%CITATION = ARXIV:0910.1106;%%
\bibitem{Ohta:1982wn}
  N.~Ohta,
  %``Grand Unified Theories Based On Local Supersymmetry,''
  Prog.\ Theor.\ Phys.\  {\bf 70}, 542 (1983).
  %%CITATION = PTPKA,70,542;%%
\bibitem{Pagels:1981ke}
  H.~Pagels and J.~R.~Primack,
  %``Supersymmetry, Cosmology And New Tev Physics,''
  Phys.\ Rev.\ Lett.\  {\bf 48}, 223 (1982).
  %%CITATION = PRLTA,48,223;%%
\bibitem{Feng:2003xh}
  J.~L.~Feng, A.~Rajaraman and F.~Takayama,
  %``Superweakly-interacting massive particles,''
  Phys.\ Rev.\ Lett.\  {\bf 91}, 011302 (2003).
  %%CITATION = PRLTA,91,011302;%%
\bibitem{Feng:2003nr}
  J.~L.~Feng, A.~Rajaraman and F.~Takayama,
  %``Graviton cosmology in universal extra dimensions,''
  Phys.\ Rev.\  D {\bf 68}, 085018 (2003).
  %%CITATION = PHRVA,D68,085018;%%
\bibitem{Rajagopal:1990yx}
  K.~Rajagopal, M.~S.~Turner and F.~Wilczek,
  %``Cosmological implications of axinos,''
  Nucl.\ Phys.\  B {\bf 358}, 447 (1991).
  %%CITATION = NUPHA,B358,447;%%
\bibitem{Covi:1999ty}
  L.~Covi, J.~E.~Kim and L.~Roszkowski,
  %``Axinos as cold dark matter,''
  Phys.\ Rev.\ Lett.\  {\bf 82}, 4180 (1999).
  %%CITATION = PRLTA,82,4180;%%
\bibitem{Covi:2001nw}
  L.~Covi, H.~B.~Kim, J.~E.~Kim and L.~Roszkowski,
  %``Axinos as dark matter,''
  JHEP {\bf 0105}, 033 (2001).
  %%CITATION = JHEPA,0105,033;%%
\bibitem{Covi:2002vw}
  L.~Covi, L.~Roszkowski and M.~Small,
  %``Effects of squark processes on the axino CDM abundance,''
  JHEP {\bf 0207}, 023 (2002).
  %%CITATION = JHEPA,0207,023;%%
\bibitem{Baer:2009ms}
  H.~Baer, A.~D.~Box and H.~Summy,
  %``Mainly axion cold dark matter in the minimal supergravity model,''
  JHEP {\bf 0908}, 080 (2009).
  %%CITATION = JHEPA,0908,080;%%
\bibitem{Asaka:2006fs}
  T.~Asaka, K.~Ishiwata and T.~Moroi,
  %``Right-handed sneutrino as cold dark matter of the universe,''
  Phys.\ Rev.\  D {\bf 75}, 065001 (2007).
  %%CITATION = PHRVA,D75,065001;%%
\bibitem{Pomarol:1999ie}
  A.~Pomarol and R.~Rattazzi,
  %``Sparticle masses from the superconformal anomaly,''
  JHEP {\bf 9905}, 013 (1999).
  %%CITATION = JHEPA,9905,013;%%
\bibitem{Choi:2005uz}
  K.~Choi, K.~S.~Jeong and K.~i.~Okumura,
  %``Phenomenology of mixed modulus-anomaly mediation in fluxed string
  %compactifications and brane models,''
  JHEP {\bf 0509}, 039 (2005).
  %%CITATION = JHEPA,0509,039;%%
\bibitem{Endo:2005uy}
  M.~Endo, M.~Yamaguchi and K.~Yoshioka,
  %``A bottom-up approach to moduli dynamics in heavy gravitino scenario:
  %Superpotential, soft terms and sparticle mass spectrum,''
  Phys.\ Rev.\  D {\bf 72}, 015004 (2005).
  %%CITATION = PHRVA,D72,015004;%%
\bibitem{Falkowski:2005ck}
  A.~Falkowski, O.~Lebedev and Y.~Mambrini,
  %``SUSY Phenomenology of KKLT Flux Compactifications,''
  JHEP {\bf 0511}, 034 (2005).
  %%CITATION = JHEPA,0511,034;%%
\bibitem{Everett:2008qy}
  L.~L.~Everett, I.~W.~Kim, P.~Ouyang and K.~M.~Zurek,
  %``Deflected Mirage Mediation: A Framework for Generalized Supersymmetry
  %Breaking,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 101803 (2008).
  %%CITATION = PRLTA,101,101803;%%
%\cite{Rattazzi:1999qg}
\bibitem{Rattazzi:1999qg}
  R.~Rattazzi, A.~Strumia and J.~D.~Wells,
  %``Phenomenology of deflected anomaly mediation,''
  Nucl.\ Phys.\  B {\bf 576}, 3 (2000).
  %%CITATION = NUPHA,B576,3;%%
\bibitem{Baer:2007eh}
  H.~Baer, E.~K.~Park, X.~Tata and T.~T.~Wang,
  %``Collider and Dark Matter Phenomenology of Models with Mirage Unification,''
  JHEP {\bf 0706}, 033 (2007).
  %%CITATION = JHEPA,0706,033;%%
\bibitem{Harrison:1982yi}
  P.~R.~Harrison and C.~H.~Llewellyn Smith,
  %``Hadroproduction Of Supersymmetric Particles,''
  Nucl.\ Phys.\  B {\bf 213}, 223 (1983)
  [Erratum-ibid.\  B {\bf 223}, 542 (1983)].
  %%CITATION = NUPHA,B213,223;%%
\bibitem{Baer:1985xz}
  H.~Baer and X.~Tata,
  %``Component Formulae For Hadroproduction Of Left-Handed And Right-Handed
  %Squarks,''
  Phys.\ Lett.\  B {\bf 160}, 159 (1985).
  %%CITATION = PHLTA,B160,159;%%
\bibitem{Barbieri:1987ed}
  R.~Barbieri, G.~Gamberini, G.~F.~Giudice and G.~Ridolfi,
  %``CONSTRAINING SUPERGRAVITY MODELS FROM GLUINO PRODUCTION,''
  Nucl.\ Phys.\  B {\bf 301}, 15 (1988).
  %%CITATION = NUPHA,B301,15;%%
\bibitem{Baer:1990sc}
  H.~Baer, X.~Tata and J.~Woodside,
  %``PHENOMENOLOGY OF GLUINO DECAYS VIA LOOPS AND TOP QUARK YUKAWA COUPLING,''
  Phys.\ Rev.\  D {\bf 42}, 1568 (1990).
  %%CITATION = PHRVA,D42,1568;%%
\bibitem{Ma:1988ns}
  E.~Ma and G.~G.~Wong,
  %``TWO-BODY RADIATIVE GLUINO DECAYS,''
  Mod.\ Phys.\ Lett.\  A {\bf 3}, 1561 (1988).
  %%CITATION = MPLAE,A3,1561;%%
\bibitem{Haber:1988px}
  H.~E.~Haber and D.~Wyler,
  %``RADIATIVE NEUTRALINO DECAY,''
  Nucl.\ Phys.\  B {\bf 323}, 267 (1989).
  %%CITATION = NUPHA,B323,267;%%
\bibitem{Komatsu:1985he}
  H.~Komatsu and J.~Kubo,
  %``The Radiative Photino Decay Into A Higgsino,''
  Phys.\ Lett.\  B {\bf 157}, 90 (1985).
  %%CITATION = PHLTA,B157,90;%%
\bibitem{Ambrosanio:1995az}
  S.~Ambrosanio and B.~Mele,
  %``Neutralino decays in the minimal supersymmetric Standard Model,''
  Phys.\ Rev.\  D {\bf 53}, 2541 (1996).
  %%CITATION = PHRVA,D53,2541;%%
\bibitem{Ambrosanio:1996gz}
  S.~Ambrosanio and B.~Mele,
  %``Supersymmetric scenarios with dominant radiative neutralino decay,''
  Phys.\ Rev.\  D {\bf 55}, 1399 (1997)
  [Erratum-ibid.\  D {\bf 56}, 3157 (1997)].
  %%CITATION = PHRVA,D55,1399;%%
\bibitem{Baer:2002kv}
  H.~Baer and T.~Krupovnickas,
  %``Radiative neutralino decay in supersymmetric models,''
  JHEP {\bf 0209}, 038 (2002).
  %%CITATION = JHEPA,0209,038;%%
\bibitem{Baer:1995nq}
  H.~Baer, C.~h.~Chen, F.~Paige and X.~Tata,
  %``Signals for minimal supergravity at the CERN large hadron collider: Multi -
  %jet plus missing energy channel,''
  Phys.\ Rev.\  D {\bf 52}, 2746 (1995).
  %%CITATION = PHRVA,D52,2746;%%
\bibitem{Abdullin:1998nv}
  S.~Abdullin and F.~Charles,
  %``Search for SUSY in (leptons +) jets + E(T)(miss) final states,''
  Nucl.\ Phys.\  B {\bf 547}, 60 (1999).
  %%CITATION = NUPHA,B547,60;%%
\bibitem{Abdullin:1998pm}
  S.~Abdullin {\it et al.}  [CMS Collaboration],
  %``Discovery potential for supersymmetry in CMS,''
  J.\ Phys.\ G {\bf 28}, 469 (2002).
  %%CITATION = JPHGB,G28,469;%%
\bibitem{Baer:1995va}
  H.~Baer, C.~h.~Chen, F.~Paige and X.~Tata,
  %``Signals for Minimal Supergravity at the CERN Large Hadron Collider II:
  %Multilepton Channels,''
  Phys.\ Rev.\  D {\bf 53}, 6241 (1996).
  %%CITATION = PHRVA,D53,6241;%%
\bibitem{Baer:1990rq}
  H.~Baer, D.~D.~Karatas and X.~Tata,
  %``GLUINO AND SQUARK PRODUCTION IN ASSOCIATION WITH GAUGINOS AT HADRON
  %SUPERCOLLIDERS,''
  Phys.\ Rev.\  D {\bf 42}, 2259 (1990).
  %%CITATION = PHRVA,D42,2259;%%
\bibitem{Baer:1993tr}
  H.~Baer, C.~Kao and X.~Tata,
  %``Aspects of chargino - neutralino production at the tevatron collider,''
  Phys.\ Rev.\  D {\bf 48}, 5175 (1993).
  %%CITATION = PHRVA,D48,5175;%%
\bibitem{Baer:1994nr}
  H.~Baer, C.~h.~Chen, F.~Paige and X.~Tata,
  %``Trileptons from chargino - neutralino production at the CERN Large Hadron
  %Collider,''
  Phys.\ Rev.\  D {\bf 50}, 4508 (1994).
  %%CITATION = PHRVA,D50,4508;%%
\bibitem{Hinchliffe:1996iu}
  I.~Hinchliffe, F.~E.~Paige, M.~D.~Shapiro, J.~Soderqvist and W.~Yao,
  %``Precision SUSY measurements at CERN LHC,''
  Phys.\ Rev.\  D {\bf 55}, 5520 (1997).
  %%CITATION = PHRVA,D55,5520;%%
\bibitem{Hinchliffe:1998ys}
  I.~Hinchliffe and F.~E.~Paige,
  %``Measurements in gauge mediated SUSY breaking models at LHC,''
  Phys.\ Rev.\  D {\bf 60}, 095002 (1999).
  %%CITATION = PHRVA,D60,095002;%%
\bibitem{Bachacou:1999zb}
  H.~Bachacou, I.~Hinchliffe and F.~E.~Paige,
  %``Measurements of masses in SUGRA models at CERN LHC,''
  Phys.\ Rev.\  D {\bf 62}, 015009 (2000).
  %%CITATION = PHRVA,D62,015009;%%
\bibitem{Barnett:1993ea}
  R.~M.~Barnett, J.~F.~Gunion and H.~E.~Haber,
  %``Discovering supersymmetry with like sign dileptons,''
  Phys.\ Lett.\  B {\bf 315}, 349 (1993).
  %%CITATION = PHLTA,B315,349;%%
\bibitem{Baer:1991xs}
  H.~Baer, X.~Tata and J.~Woodside,
  %``Multi - lepton signals from supersymmetry at hadron super colliders,''
  Phys.\ Rev.\  D {\bf 45}, 142 (1992).
  %%CITATION = PHRVA,D45,142;%%
\bibitem{Baer:2000pe}
  H.~Baer, P.~G.~Mercadante, X.~Tata and Y.~l.~Wang,
  %``The Reach of the CERN large hadron collider for gauge mediated
  %supersymmetry breaking models,''
  Phys.\ Rev.\  D {\bf 62}, 095007 (2000).
  %%CITATION = PHRVA,D62,095007;%%
\bibitem{Baer:1997yi}
  H.~Baer, C.~h.~Chen, M.~Drees, F.~Paige and X.~Tata,
  %``Collider phenomenology for supersymmetry with large tan Beta,''
  Phys.\ Rev.\ Lett.\  {\bf 79}, 986 (1997)
  [Erratum-ibid.\  {\bf 80}, 642 (1998)].
  %%CITATION = PRLTA,79,986;%%
\bibitem{Baer:1998kt}
  H.~Baer, P.~G.~Mercadante and X.~Tata,
  %``Searching for bottom squarks at luminosity upgrades of the Fermilab
  %Tevatron,''
  Phys.\ Rev.\  D {\bf 59}, 015010 (1999).
  %%CITATION = PHRVA,D59,015010;%%
\bibitem{Chattopadhyay:2000qa}
  U.~Chattopadhyay, A.~Datta, A.~Datta, A.~Datta and D.~P.~Roy,
  %``LHC signature of the minimal SUGRA model with a large soft scalar mass,''
  Phys.\ Lett.\  B {\bf 493}, 127 (2000).
  %%CITATION = PHLTA,B493,127;%%
\bibitem{Mercadante:2005vx}
  P.~G.~Mercadante, J.~K.~Mizukoshi and X.~Tata,
  %``Using b-tagging to enhance the SUSY reach of the CERN Large Hadron
  %Collider,''
  Phys.\ Rev.\  D {\bf 72}, 035009 (2005).
  %%CITATION = PHRVA,D72,035009;%%
\bibitem{Das:2007jn}
  S.~P.~Das, A.~Datta, M.~Guchait, M.~Maity and S.~Mukherjee,
  %``Focus Point SUSY at the LHC Revisited,''
  Eur.\ Phys.\ J.\  C {\bf 54}, 645 (2008).
  %%CITATION = EPHJA,C54,645;%%
\bibitem{Kadala:2008uy}
  R.~H.~K.~Kadala, P.~G.~Mercadante, J.~K.~Mizukoshi and X.~Tata,
  %``Heavy-flavour tagging and the supersymmetry reach of the CERN Large Hadron
  %Collider,''
  Eur.\ Phys.\ J.\  C {\bf 56}, 511 (2008).
  %%CITATION = EPHJA,C56,511;%%
\bibitem{Baer:1990in}
  H.~Baer, X.~Tata and J.~Woodside,
  %``$Z^0$ + JETS + (missing) $p_{T}$ EVENTS AS A SIGNAL FOR SUPERSYMMETRY AT
  %THE TEVATRON COLLIDER,''
  Phys.\ Rev.\  D {\bf 42}, 1450 (1990).
  %%CITATION = PHRVA,D42,1450;%%
\bibitem{Baer:1992ef}
  H.~Baer, M.~Bisset, X.~Tata and J.~Woodside,
  %``Supercollider signals from gluino and squark decays to Higgs bosons,''
  Phys.\ Rev.\  D {\bf 46}, 303 (1992).
  %%CITATION = PHRVA,D46,303;%%
\bibitem{Baer:1992kd}
  H.~Baer, M.~Bisset, D.~Dicus, C.~Kao and X.~Tata,
  %``The Search for Higgs bosons of minimal supersymmetry: Impact of
  %supersymmetric decay modes,''
  Phys.\ Rev.\  D {\bf 47}, 1062 (1993).
  %%CITATION = PHRVA,D47,1062;%%
\bibitem{Baer:1994fx}
  H.~Baer, M.~Bisset, C.~Kao and X.~Tata,
  %``Detecting Higgs boson decays to neutralinos at hadron supercolliders,''
  Phys.\ Rev.\  D {\bf 50}, 316 (1994).
  %%CITATION = PHRVA,D50,316;%%
\bibitem{Moortgat:2001pp}
  F.~Moortgat, S.~Abdullin and D.~Denegri,
  %``Observability of MSSM Higgs bosons via sparticle decay modes in CMS,''
  arXiv:hep-ph/0112046.
  %%CITATION = HEP-PH/0112046;%%
\bibitem{Bisset:2007mi}
  M.~Bisset, J.~Li, N.~Kersting, F.~Moortgat and S.~Moretti,
  %``Four-lepton LHC events from MSSM Higgs boson decays into neutralino and
  %chargino pairs,''
  JHEP {\bf 0908}, 037 (2009).
  %%CITATION = JHEPA,0908,037;%%
\bibitem{Baer:1993ew}
  H.~Baer, C.~h.~Chen, F.~Paige and X.~Tata,
  %``Detecting sleptons at hadron colliders and supercolliders,''
  Phys.\ Rev.\  D {\bf 49}, 3283 (1994).
  %%CITATION = PHRVA,D49,3283;%%
\bibitem{Barr:2005dz}
  A.~J.~Barr,
  %``Measuring slepton spin at the LHC,''
  JHEP {\bf 0602}, 042 (2006).
  %%CITATION = JHEPA,0602,042;%%
\bibitem{Baer:1994nr}
  H.~Baer, C.~h.~Chen, F.~Paige and X.~Tata,
  %``Trileptons from chargino - neutralino production at the CERN Large Hadron
  %Collider,''
  Phys.\ Rev.\  D {\bf 50}, 4508 (1994).
  %%CITATION = PHRVA,D50,4508;%%
\bibitem{Dimopoulos:1996yq}
  S.~Dimopoulos, S.~D.~Thomas and J.~D.~Wells,
  %``Sparticle spectroscopy and electroweak symmetry breaking with
  %gauge-mediated supersymmetry breaking,''
  Nucl.\ Phys.\  B {\bf 488}, 39 (1997).
  %%CITATION = NUPHA,B488,39;%%
\bibitem{Baer:1998ve}
  H.~Baer, P.~G.~Mercadante, F.~Paige, X.~Tata and Y.~Wang,
  %``LHC reach for gauge mediated supersymmetry breaking models via prompt
  %photon channels,''
  Phys.\ Lett.\  B {\bf 435}, 109 (1998).
  %%CITATION = PHLTA,B435,109;%%
\bibitem{Baer:2005jq}
  H.~Baer, T.~Krupovnickas, A.~Mustafayev, E.~K.~Park, S.~Profumo and X.~Tata,
  %``Exploring the BWCA (Bino-Wino co-annihilation) scenario for neutralino
  %dark matter,''
  JHEP {\bf 0512}, 011 (2005).
  %%CITATION = JHEPA,0512,011;%%
\bibitem{Baer:2003wx}
  H.~Baer, C.~Balazs, A.~Belyaev, T.~Krupovnickas and X.~Tata,
  %``Updated reach of the CERN LHC and constraints from relic density, $b \to s
  %\gamma$ and a($\mu$) in the mSUGRA model,''
  JHEP {\bf 0306}, 054 (2003).
  %%CITATION = JHEPA,0306,054;%%
\bibitem{Ambrosanio:2000ik}
  S.~Ambrosanio, B.~Mele, S.~Petrarca, G.~Polesello and A.~Rimoldi,
  %``Measuring the SUSY breaking scale at the LHC in the slepton NLSP  scenario
  %of GMSB models,''
  JHEP {\bf 0101}, 014 (2001).
  %%CITATION = JHEPA,0101,014;%%
\bibitem{Hamaguchi:2007ji}
  K.~Hamaguchi, S.~Shirai and T.~T.~Yanagida,
  %``Determining the mass for an ultralight gravitino at LHC,''
  Phys.\ Lett.\  B {\bf 663}, 86 (2008).
  %%CITATION = PHLTA,B663,86;%%
\bibitem{Feng:2004yi}
  J.~L.~Feng and B.~T.~Smith,
  %``Slepton trapping at the Large Hadron and International Linear  Colliders,''
  Phys.\ Rev.\  D {\bf 71}, 015004 (2005)
  [Erratum-ibid.\  D {\bf 71}, 019904 (2005)].
  %%CITATION = PHRVA,D71,015004;%%
\bibitem{Hamaguchi:2006vu}
  K.~Hamaguchi, M.~M.~Nojiri and A.~de Roeck,
  %``Prospects to study a long-lived charged next lightest supersymmetric
  %particle at the LHC,''
  JHEP {\bf 0703}, 046 (2007).
  %%CITATION = JHEPA,0703,046;%%
\bibitem{Hamaguchi:2004df}
  K.~Hamaguchi, Y.~Kuno, T.~Nakaya and M.~M.~Nojiri,
  %``A study of late decaying charged particles at future colliders,''
  Phys.\ Rev.\  D {\bf 70}, 115007 (2004).
  %%CITATION = PHRVA,D70,115007;%%
\bibitem{Asai:2009ka}
  S.~Asai, K.~Hamaguchi and S.~Shirai,
  %``Stop and Decay of Long-lived Charged Massive Particles at the LHC
  %detectors,''
  Phys.\ Rev.\ Lett.\  {\bf 103}, 141803 (2009).
  %%CITATION = PRLTA,103,141803;%%
\bibitem{Kawagoe:2003jv}
  K.~Kawagoe, T.~Kobayashi, M.~M.~Nojiri and A.~Ochi,
  %``Study of the gauge mediation signal with non-pointing photons at the  CERN
  %LHC,''
  Phys.\ Rev.\  D {\bf 69}, 035003 (2004).
  %%CITATION = PHRVA,D69,035003;%%
\bibitem{Baer:1998pg}
  H.~Baer, K.~m.~Cheung and J.~F.~Gunion,
  %``A Heavy gluino as the lightest supersymmetric particle,''
  Phys.\ Rev.\  D {\bf 59}, 075002 (1999).
  %%CITATION = PHRVA,D59,075002;%%
\bibitem{ArkaniHamed:2004fb}
  N.~Arkani-Hamed and S.~Dimopoulos,
  %``Supersymmetric unification without low energy supersymmetry and  signatures
  %for fine-tuning at the LHC,''
  JHEP {\bf 0506}, 073 (2005).
  %%CITATION = JHEPA,0506,073;%%
\bibitem{ArkaniHamed:2004yi}
  N.~Arkani-Hamed, S.~Dimopoulos, G.~F.~Giudice and A.~Romanino,
  %``Aspects of split supersymmetry,''
  Nucl.\ Phys.\  B {\bf 709}, 3 (2005).
  %%CITATION = NUPHA,B709,3;%%
\bibitem{Kilian:2004uj}
  W.~Kilian, T.~Plehn, P.~Richardson and E.~Schmidt,
  %``Split supersymmetry at colliders,''
  Eur.\ Phys.\ J.\  C {\bf 39}, 229 (2005).
  %%CITATION = EPHJA,C39,229;%%
\bibitem{Drees:1990yw}
  M.~Drees and X.~Tata,
  %``Signals for heavy exotics at hadron colliders and supercolliders,''
  Phys.\ Lett.\  B {\bf 252}, 695 (1990).
  %%CITATION = PHLTA,B252,695;%%
\bibitem{Baer:1996wa}
  H.~Baer, C.~h.~Chen and X.~Tata,
  %``Impact of hadronic decays of the lightest neutralino on the reach of  the
  %CERN LHC,''
  Phys.\ Rev.\  D {\bf 55}, 1466 (1997).
  %%CITATION = PHRVA,D55,1466;%%
\bibitem{Baer:1994zw}
  H.~Baer, C.~Kao and X.~Tata,
  %``Impact of R-parity violation on supersymmetry searches at the tevatron,''
  Phys.\ Rev.\  D {\bf 51}, 2180 (1995).
  %%CITATION = PHRVA,D51,2180;%%
\bibitem{Choudhury:2002av}
  D.~Choudhury, R.~M.~Godbole and G.~Polesello,
  %``Measuring R parity violating couplings in dilepton production at the LHC,''
  JHEP {\bf 0208}, 004 (2002).
  %%CITATION = JHEPA,0208,004;%%
\bibitem{Bartl:1996cg}
  A.~Bartl, W.~Porod, F.~de Campos, M.~A.~Garcia-Jareno, M.~B.~Magro, J.~W.~F.~Valle and W.~Majerotto,
  %``Signatures of spontaneous breaking of R-parity in gluino cascade decays at
  %LHC,''
  Nucl.\ Phys.\  B {\bf 502}, 19 (1997).
  %%CITATION = NUPHA,B502,19;%%
\bibitem{Dimopoulos:1988jw}
  S.~Dimopoulos and L.~J.~Hall,
  %``Lepton and Baryon Number Violating Collider Signatures from
  %Supersymmetry,''
  Phys.\ Lett.\  B {\bf 207}, 210 (1988).
  %%CITATION = PHLTA,B207,210;%%
\bibitem{Dreiner:2008rv}
  H.~K.~Dreiner, S.~Grab and M.~K.~Trenkel,
  %``$S\tau$ LSP Phenomenology: Two versus Four-Body Decay Modes. Example:
  %Resonant Single Slepton Production at the LHC,''
  Phys.\ Rev.\  D {\bf 79}, 016002 (2009)
  [Erratum-ibid.\  {\bf 79}, 019902 (2009)].
  %%CITATION = PHRVA,D79,016002;%%
\bibitem{Bernhardt:2008jz}
  M.~A.~Bernhardt, S.~P.~Das, H.~K.~Dreiner and S.~Grab,
  %``Sneutrino as Lightest Supersymmetric Particle in $B_{3}$ mSUGRA Models and
  %Signals at the LHC,''
  Phys.\ Rev.\  D {\bf 79}, 035003 (2009).
  %%CITATION = PHRVA,D79,035003;%%
\bibitem{Bornhauser:2009ru}
  S.~Bornhauser, M.~Drees, H.~K.~Dreiner and J.~S.~Kim,
  %``Rapidity Gap Events in Squark Pair Production at the LHC,''
  Phys.\ Rev.\  D {\bf 80}, 095007 (2009).
  %%CITATION = PHRVA,D80,095007;%%
\bibitem{Bornhauser:2009av}
  S.~Bornhauser, M.~Drees, H.~K.~Dreiner and J.~S.~Kim,
  %``Rapidity Gap Events for Squark Pair Production at the LHC,''
  arXiv:0909.5155 [hep-ph].
  %%CITATION = ARXIV:0909.5155;%%
\bibitem{Allanach:2002nj}
  B.~C.~Allanach {\it et al.},
  %``The Snowmass points and slopes: Benchmarks for SUSY searches,''
%in {\it Proc. of the APS/DPF/DPB Summer Study on the Future of
%Particle Physics (Snowmass 2001) } ed. N.~Graf,
  Eur.\ Phys.\ J.\  C {\bf 25}, 113 (2002).
  %%CITATION = EPHJA,C25,113;%%
\bibitem{Weiglein:2004hn}
  G.~Weiglein {\it et al.}  [LHC/LC Study Group],
  %``Physics interplay of the LHC and the ILC,''
  Phys.\ Rept.\  {\bf 426}, 47 (2006).
  %%CITATION = PRPLC,426,47;%%
\bibitem{Djouadi:2002ze}
  A.~Djouadi, J.~L.~Kneur and G.~Moultaka,
  %``SuSpect: A Fortran code for the supersymmetric and Higgs particle spectrum
  %in the MSSM,''
  Comput.\ Phys.\ Commun.\  {\bf 176}, 426 (2007).
  %%CITATION = CPHCB,176,426;%%
\bibitem{Hocker:2001xe}
  A.~Hocker, H.~Lacker, S.~Laplace and F.~Le Diberder,
  %``A New approach to a global fit of the CKM matrix,''
  Eur.\ Phys.\ J.\  C {\bf 21}, 225 (2001).
  %%CITATION = EPHJA,C21,225;%%
\bibitem{:2008gva}
  M.~M.~Nojiri {\it et al.},
  %``Physics Beyond the Standard Model: Supersymmetry,''
  arXiv:0802.3672 [hep-ph].
  %%CITATION = ARXIV:0802.3672;%%
%%%%%%%%%%%
\bibitem{AbdusSalam:2009qd}
  S.~S.~AbdusSalam, B.~C.~Allanach, F.~Quevedo, F.~Feroz and M.~Hobson,
  %``Fitting the Phenomenological MSSM,''
  arXiv:0904.2548 [hep-ph].
  %%CITATION = ARXIV:0904.2548;%%
\bibitem{Feroz:2007kg}
  F.~Feroz and M.~P.~Hobson,
  %``Multimodal nested sampling: an efficient and robust alternative to MCMC
  %methods for astronomical data analysis,''
  arXiv:0704.3704 [astro-ph].
  %%CITATION = ARXIV:0704.3704;%%
\bibitem{Feroz:2008xx}
  F.~Feroz, M.~P.~Hobson and M.~Bridges,
  %``MultiNest: an efficient and robust Bayesian inference tool for cosmology
  %and particle physics,''
  arXiv:0809.3437 [astro-ph].
  %%CITATION = ARXIV:0809.3437;%%
\bibitem{Skands:2003cj}
  P.~Z.~Skands {\it et al.},
  %``SUSY Les Houches Accord: Interfacing SUSY Spectrum Calculators, Decay
  %Packages, and Event Generators,''
  JHEP {\bf 0407}, 036 (2004).
  %%CITATION = JHEPA,0407,036;%%
\bibitem{Allanach:2001kg}
  B.~C.~Allanach,
  %``SOFTSUSY: A C++ program for calculating supersymmetric spectra,''
  Comput.\ Phys.\ Commun.\  {\bf 143}, 305 (2002).
  %%CITATION = CPHCB,143,305;%%
\bibitem{Belanger:2004yn}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``micrOMEGAs: Version 1.3,''
  Comput.\ Phys.\ Commun.\  {\bf 174}, 577 (2006).
  %%CITATION = CPHCB,174,577;%%
\bibitem{Mahmoudi:2008tp}
  F.~Mahmoudi,
  %``SuperIso v2.3: A Program for calculating flavor physics observables in
  %Supersymmetry,''
  Comput.\ Phys.\ Commun.\  {\bf 180}, 1579 (2009).
  %%CITATION = CPHCB,180,1579;%%
\bibitem{Heinemeyer:2007bw}
  S.~Heinemeyer, W.~Hollik, A.~M.~Weber and G.~Weiglein,
  %``$Z$ Pole Observables in the MSSM,''
  JHEP {\bf 0804}, 039 (2008).
  %%CITATION = JHEPA,0804,039;%%
\bibitem{AbdusSalam:2008uv}
  S.~S.~AbdusSalam,
  %``The Full 24-Parameter MSSM Exploration,''
  AIP Conf.\ Proc.\  {\bf 1078}, 297 (2009).
  %%CITATION = APCPC,1078,297;%%
\bibitem{Lebedev:2005ge}
  O.~Lebedev, H.~P.~Nilles and M.~Ratz,
  %``A note on fine-tuning in mirage mediation,''
  arXiv:hep-ph/0511320.
  %%CITATION = HEP-PH/0511320;%%
\bibitem{Conlon:2006wz}
  J.~P.~Conlon, S.~S.~Abdussalam, F.~Quevedo and K.~Suruliz,
  %``Soft SUSY breaking terms for chiral matter in IIB string
  %compactifications,''
  JHEP {\bf 0701}, 032 (2007).
  %%CITATION = JHEPA,0701,032;%%
\bibitem{Conlon:2006us}
  J.~P.~Conlon and F.~Quevedo,
  %``Gaugino and scalar masses in the landscape,''
  JHEP {\bf 0606}, 029 (2006).
  %%CITATION = JHEPA,0606,029;%%
\bibitem{Conlon:2007xv}
  J.~P.~Conlon, C.~H.~Kom, K.~Suruliz, B.~C.~Allanach and F.~Quevedo,
  %``Sparticle Spectra and LHC Signatures for Large Volume String
  %Compactifications,''
  JHEP {\bf 0708}, 061 (2007).
  %%CITATION = JHEPA,0708,061;%%
\bibitem{DeRoeck:2009id}
  A.~De Roeck {\it et al.},
  %``From the LHC to Future Colliders,''
  arXiv:0909.3240 [hep-ph].
  %%CITATION = ARXIV:0909.3240;%%
\bibitem{Lester:1999tx}
  C.~G.~Lester and D.~J.~Summers,
  %``Measuring masses of semiinvisibly decaying particles pair produced at
  %hadron colliders,''
  Phys.\ Lett.\  B {\bf 463}, 99 (1999).
  %%CITATION = PHLTA,B463,99;%%
\bibitem{Barr:2003rg}
  A.~Barr, C.~Lester and P.~Stephens,
  %``m(T2) : The Truth behind the glamour,''
  J.\ Phys.\ G {\bf 29}, 2343 (2003).
  %%CITATION = JPHGB,G29,2343;%%
\bibitem{Cho:2007qv}
  W.~S.~Cho, K.~Choi, Y.~G.~Kim and C.~B.~Park,
  %``Gluino Stransverse Mass,''
  Phys.\ Rev.\ Lett.\  {\bf 100}, 171801 (2008).
  %%CITATION = PRLTA,100,171801;%%
\bibitem{Cho:2007dh}
  W.~S.~Cho, K.~Choi, Y.~G.~Kim and C.~B.~Park,
  %``Measuring superparticle masses at hadron collider using the transverse mass
  %kink,''
  JHEP {\bf 0802}, 035 (2008).
  %%CITATION = JHEPA,0802,035;%%
\bibitem{Gripaios:2007is}
  B.~Gripaios,
  %``Transverse Observables and Mass Determination at Hadron Colliders,''
  JHEP {\bf 0802}, 053 (2008).
  %%CITATION = JHEPA,0802,053;%%
\bibitem{Barr:2007hy}
  A.~J.~Barr, B.~Gripaios and C.~G.~Lester,
  %``Weighing Wimps with Kinks at Colliders: Invisible Particle Mass
  %Measurements from Endpoints,''
  JHEP {\bf 0802}, 014 (2008).
  %%CITATION = JHEPA,0802,014;%%
\bibitem{Cho:2008tj}
  W.~S.~Cho, K.~Choi, Y.~G.~Kim and C.~B.~Park,
  %``M_T2-assisted on-shell reconstruction of missing momenta and its
  %application to spin measurement at the LHC,''
  Phys.\ Rev.\  D {\bf 79}, 031701 (2009).
  %%CITATION = PHRVA,D79,031701;%%
\bibitem{Choi:2009hn}
  K.~Choi, S.~Choi, J.~S.~Lee and C.~B.~Park,
  %``Reconstructing the Higgs boson in dileptonic W decays at hadron collider,''
  Phys.\ Rev.\  D {\bf 80}, 073010 (2009).
  %%CITATION = PHRVA,D80,073010;%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% (3) HIGGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

